Optimal Algorithms for Mean Estimation under Local Differential Privacy

We study the problem of mean estimation of $\ell_2$-bounded vectors under the constraint of local differential privacy. While the literature has a variety of algorithms that achieve the asymptotically optimal rates for this problem, the performance of these algorithms in practice can vary significantly due to varying (and often large) hidden constants. In this work, we investigate the question of designing the protocol with the smallest variance. We show that PrivUnit (Bhowmick et al. 2018) with optimized parameters achieves the optimal variance among a large family of locally private randomizers. To prove this result, we establish some properties of local randomizers, and use symmetrization arguments that allow us to write the optimal randomizer as the optimizer of a certain linear program. These structural results, which should extend to other problems, then allow us to show that the optimal randomizer belongs to the PrivUnit family. We also develop a new variant of PrivUnit based on the Gaussian distribution which is more amenable to mathematical analysis and enjoys the same optimality guarantees. This allows us to establish several useful properties on the exact constants of the optimal error as well as to numerically estimate these constants.

==> alg-proj.tex <==


% \section{$k$-Projection PrivUnit: near optimal rates with compression}
% \label{sec:alg-proj}

%\ha{complete}



==> experiments-paper.tex <==


\section{Experiments}
\label{sec:exp}

\ha{complete}

==> experiments.tex <==

\section{Algorithms and Experiments}


Let us begin by describing the family of algorithms we consider for $\diffp \ge 1$ which are variants and extensions of $\privunit_2$ and $\djw$.

\subsection{Repetition-based Algorithms}
In this scheme, we apply the algorithm $k = \diffp$ times and report the mean of these runs. This is easily applicable to both $\privunit_2$ and $\djw$ and gives asymptotically optimal bounds.

\subsection{Chunking-based Algorithms}
Instead of repeating the algorithms $k$ times, these algorithms divide the vectors to $k$ different chunks and apply an $\frac{\diffp}{k}$-DP versions of the algorithms we have for each chunk.

\subsection{Projection-based Algorithms}
These algorithms proceed by projecting the input vector to a $k$-dimensional subspace then privatizing the signs of the $k$-dimensional vector. More precisely, these algorithms work as follows:
\begin{enumerate}
    \item (Potentially) Rotate the input vector $v$
    \item Pick $k$ vectors $\{u_1,\dots,u_k\} \in \sphere_2^d$
    \item Privatize $(s_1,\dots,s_k)$ where $s_i = \text{sign}(\<v,u_i \>)$ to get $(\hat s_1,\dots,\hat s_k)$
    \item Return $C \sum_{i=1}^k \hat s_i u_i$
\end{enumerate}
where $C$ is a normalization constant. Note that these methods have different behavior depending on the algorithms chosen in steps 1 and 2. For step 1, we will consider different choices of the vectors such as
\begin{enumerate}
    \item Random vectors: sample $u_1,\dots,u_k \simiid \mathsf{Unif} (\sphere_2^d)$
    \item Random orthogonal vectors: sample random orthogonal unit vectors $u_1,\dots,u_k$ such that $\<u_i,u_j\>=0$.
    \item (Deterministic) Chunk-based random vectors: define $k$ chunks $B_1,\dots,B_k$ of size $m=\frac{d}{k}$ and sample vectors $u_1,\dots,u_k$ such that for all $i \in [k]$, $u_{i,B_i} \sim \mathsf{Unif}(\sphere_2^m)$ and $u_{i,[d] \setminus B_i} = 0$. \ha{problem here: need to know norm of chunks to make estimate unbiased}
    \item (Random) Chunk-based random vectors: same as the previous one, however here we sample a random set of indices for each chunk independently. That is, to sample $u_i$, we first sample a random set $B_i$ of size $m$ from $[d]$ then we sample $u_i$ using $u_{i,B_i} \sim \mathsf{Unif}(\sphere_2^m)$ and $u_{i,[d] \setminus B_i} = 0$. 
\end{enumerate}
random vectors, random $1$-sparse vectors,  chunk-based random vectors. 
For step 2, we mainly consider
\begin{enumerate}
    \item $\rr$: apply $2^k$-Randomized Response to the signs $(s_1,\dots,s_k)$.
    \item $\privunit_\infty$: apply $\privunit_\infty$ to the signs $(s_1,\dots,s_k)$~\cite{BhowmickDuFrKaRo18}.
\end{enumerate}

Let us now discuss the normalization constant.
To calculate $C$, assume for now that the $u_i$'s has the same distribution. Then we have
\begin{align*}
    \E[\hat v]
         = C k \E[\hat s_i u_i]
\end{align*}
The algorithms we consider for privatizing the signs $\R$ can be written as $\R(s_1,\dots,s_k) = \R(\mathbf{1}) s$ hence we can write $\hat s_i = \R_i(\mathbf{1}) s_i$. Using this, we now have
\begin{align*}
   \E[\hat s_i u_i]
        & = \E[\R_i(\mathbf{1}) s_i u_i] \\
        & = \E[\R_i(\mathbf{1}) ] \cdot \E[s_i u_i] .%\\
        %& = (2p_{\mathsf{correct}} - 1 ) \cdot \E[s_i u_i]\\
        %& = (2p_{\mathsf{correct}} - 1 ) \cdot \E[u_i \mid \<v,u_i\> \ge 0],
\end{align*}
%where $p_{\mathsf{correct}} = P_{\R}(\R_i(\mathbf{1})=1)$.
We can therefore take care of each of these term separately. Note that for $\privunit_\infty$ we have $\E[\privunit_\infty(\mathbf{1})] = \mathbf{1}$ and for $2^k-\rr$ we have
\begin{align*}
   \E[\R_i(\mathbf{1}) ] = (2p_{\mathsf{correct}} - 1 ) ,
\end{align*}
where $p_{\mathsf{correct}} = P_{\R}(\R_i(\mathbf{1})=1)$ is the probability of correct sign and is equal to
\begin{align*}
   p_{\mathsf{correct}}
    = \frac{e^{\diffp}}{e^{\diffp} + 2^k -1}
      + \frac{2^{k-1} - 1}{e^{\diffp} + 2^k -1}. %\frac{2^{k-1} - 1}{2^k - 1}.
\end{align*}

As for the second term, note that if $u_i$ are drawn randomly from the sphere then
\begin{align*}
   \E[s_i u_i] 
        & = \E[u_i \mid \<u_i,v\> \ge 0] \\
        & = \E[u_{i,1} \mid u_{i,1} \ge 0],
\end{align*}
for which we have an exact formula.

If the $u_i$ are drawn independently on different chunks, then looking at the first chunk $B_1$ we have
\begin{align*}
   \E[s_1 u_1] 
        & = \E[\sign(\<v_{B_1},u_1\>) u_1] \\
        & = \E[u_1 \mid \<v_{B_1},u_1\> \ge 0] ,
\end{align*}
which again we can calculate. \ha{here we need to know $\ltwo{v_{B_1}}$ to make this unbiased? if the $B_i$'s are random we can take care of this. otherwise not sure}



\subsection{Experiments}

Let us start with some experiments for repetition and chunking based algorithms in~\Cref{fig:rep-chunk}.


% \begin{figure}[t]
%   \begin{center}
%     \begin{tabular}{ccc}
%       \begin{overpic}[width=.34\columnwidth]{%,grid]{
%       {plots/LDP_rep_chunk_4.0_d=32}.pdf}
%       \end{overpic} &
%       \hspace{-1cm}
%       \begin{overpic}[width=.34\columnwidth]{%,grid]{
%     {plots/LDP_rep_chunk_8.0_d=32}.pdf}
%       \end{overpic} &
%       \hspace{-1cm}
%       \begin{overpic}[width=.34\columnwidth]{%,grid]{
% 	  {plots/LDP_rep_chunk_16.0_d=32}.pdf}
%       \end{overpic}
%       \\
%       (a) & (b)  & (c)
%     \end{tabular}
%     \caption{\label{fig:rep-chunk-small-d} Performance of Repetition and chunking based algorithms for $d=32$.}
%   \end{center}
% \end{figure}


\begin{figure}[t]
  \begin{center}
    \begin{tabular}{ccc}
      \begin{overpic}[width=.34\columnwidth]{%,grid]{
      {plots/LDP_rep_chunk_4.0_d=32}.pdf}
      \end{overpic} &
      \hspace{-1cm}
      \begin{overpic}[width=.34\columnwidth]{%,grid]{
    {plots/LDP_rep_chunk_8.0_d=32}.pdf}
      \end{overpic} &
      \hspace{-1cm}
      \begin{overpic}[width=.34\columnwidth]{%,grid]{
	  {plots/LDP_rep_chunk_16.0_d=32}.pdf}
      \end{overpic}
      \\
      (a) & (b)  & (c)
    \end{tabular}
    %\caption{\label{fig:rep-chunk-small-d} Performance of Repetition and chunking based algorithms for $d=32$.}
  \end{center}
  
  \begin{center}
    \begin{tabular}{ccc}
      \begin{overpic}[width=.34\columnwidth]{%,grid]{
      {plots/LDP_rep_chunk_4.0_d=64}.pdf}
      \end{overpic} &
      \hspace{-1cm}
      \begin{overpic}[width=.34\columnwidth]{%,grid]{
    {plots/LDP_rep_chunk_8.0_d=64}.pdf}
      \end{overpic} &
      \hspace{-1cm}
      \begin{overpic}[width=.34\columnwidth]{%,grid]{
	  {plots/LDP_rep_chunk_16.0_d=64}.pdf}
      \end{overpic}
      \\
      (a) & (b)  & (c)
    \end{tabular}
    \caption{\label{fig:rep-chunk} Performance of Repetition and chunking based algorithms for $d=32$ and $d=64$ in the top and bottom row, respectively.}
  \end{center}
\end{figure}



Let us now evaluate the performance of projection-based methods. We being in~\Cref{fig:rand-proj} where we plot the error for algorithms based on random projections with $\rr$ or $\privunit_\infty$ for privatizing the signs. We also plot the performance for the ``noiseless'' algorithm that uses the exact signs. In~\Cref{fig:rand-chunk-proj} we show the same plots when the projections are based on random vectors over (deterministic) chunks.



\begin{figure}[t]
  \begin{center}
    \begin{tabular}{ccc}
      \begin{overpic}[width=.34\columnwidth]{%,grid]{
      {plots/LDP_prj_rand_eps=4.0_d=32}.pdf}
      \end{overpic} &
      \hspace{-1cm}
      \begin{overpic}[width=.34\columnwidth]{%,grid]{
    {plots/LDP_prj_rand_eps=8.0_d=32}.pdf}
      \end{overpic} &
      \hspace{-1cm}
      \begin{overpic}[width=.34\columnwidth]{%,grid]{
	  {plots/LDP_prj_rand_eps=16.0_d=32}.pdf}
      \end{overpic}
      \\
      (a) & (b)  & (c)
    \end{tabular}
    %\caption{\label{fig:rand-proj} Performance of Projection-based algorithms with random projections and $d=32$.}
  \end{center}

  \begin{center}
    \begin{tabular}{ccc}
      \begin{overpic}[width=.34\columnwidth]{%,grid]{
      {plots/LDP_prj_rand_eps=4.0_d=64}.pdf}
      \end{overpic} &
      \hspace{-1cm}
      \begin{overpic}[width=.34\columnwidth]{%,grid]{
    {plots/LDP_prj_rand_eps=8.0_d=64}.pdf}
      \end{overpic} &
      \hspace{-1cm}
      \begin{overpic}[width=.34\columnwidth]{%,grid]{
	  {plots/LDP_prj_rand_eps=16.0_d=64}.pdf}
      \end{overpic}
      \\
      (a) & (b)  & (c)
    \end{tabular}
    \caption{\label{fig:rand-proj} Performance of Projection-based algorithms with random projections for $d=32$ and $d=64$ in the top and bottom row, respectively.}
  \end{center}


\end{figure}



% \begin{figure}[t]
%   \begin{center}
%     \begin{tabular}{ccc}
%       \begin{overpic}[width=.34\columnwidth]{%,grid]{
%       {plots/LDP_prj_rand_orth_eps=4.0_d=32}.pdf}
%       \end{overpic} &
%       \hspace{-1cm}
%       \begin{overpic}[width=.34\columnwidth]{%,grid]{
%     {plots/LDP_prj_rand_orth_eps=8.0_d=32}.pdf}
%       \end{overpic} &
%       \hspace{-1cm}
%       \begin{overpic}[width=.34\columnwidth]{%,grid]{
% 	  {plots/LDP_prj_rand_orth_eps=16.0_d=32}.pdf}
%       \end{overpic}
%       \\
%       (a) & (b)  & (c)
%     \end{tabular}
%     %\caption{\label{fig:rand-proj} Performance of Projection-based algorithms with random projections and $d=32$.}
%   \end{center}

%   \begin{center}
%     \begin{tabular}{ccc}
%       \begin{overpic}[width=.34\columnwidth]{%,grid]{
%       {plots/LDP_prj_rand_orth_eps=4.0_d=64}.pdf}
%       \end{overpic} &
%       \hspace{-1cm}
%       \begin{overpic}[width=.34\columnwidth]{%,grid]{
%     {plots/LDP_prj_rand_orth_eps=8.0_d=64}.pdf}
%       \end{overpic} &
%       \hspace{-1cm}
%       \begin{overpic}[width=.34\columnwidth]{%,grid]{
% 	  {plots/LDP_prj_rand_orth_eps=16.0_d=64}.pdf}
%       \end{overpic}
%       \\
%       (a) & (b)  & (c)
%     \end{tabular}
%     \caption{\label{fig:rand-proj} Performance of Projection-based algorithms with random orthogonal projections for $d=32$ and $d=64$ in the top and bottom row, respectively.}
%   \end{center}


% \end{figure}



\begin{figure}[t]
  \begin{center}
    \begin{tabular}{ccc}
      \begin{overpic}[width=.34\columnwidth]{%,grid]{
      {plots/LDP_prj_rand_ortheps=4.0_d=32}.pdf}
      \end{overpic} &
      \hspace{-1cm}
      \begin{overpic}[width=.34\columnwidth]{%,grid]{
    {plots/LDP_prj_rand_ortheps=8.0_d=32}.pdf}
      \end{overpic} &
      \hspace{-1cm}
      \begin{overpic}[width=.34\columnwidth]{%,grid]{
	  {plots/LDP_prj_rand_ortheps=16.0_d=32}.pdf}
      \end{overpic}
      \\
      (a) & (b)  & (c)
    \end{tabular}
    %\caption{\label{fig:rand-proj} Performance of Projection-based algorithms with random projections and $d=32$.}
  \end{center}

  \begin{center}
    \begin{tabular}{ccc}
      \begin{overpic}[width=.34\columnwidth]{%,grid]{
      {plots/LDP_prj_rand_ortheps=4.0_d=64}.pdf}
      \end{overpic} &
      \hspace{-1cm}
      \begin{overpic}[width=.34\columnwidth]{%,grid]{
    {plots/LDP_prj_rand_ortheps=8.0_d=64}.pdf}
      \end{overpic} &
      \hspace{-1cm}
      \begin{overpic}[width=.34\columnwidth]{%,grid]{
	  {plots/LDP_prj_rand_ortheps=16.0_d=64}.pdf}
      \end{overpic}
      \\
      (a) & (b)  & (c)
    \end{tabular}
    \caption{\label{fig:rand-chunk-proj} Performance of Projection-based algorithms with random orthogonal projections for $d=32$ and $d=64$ in the top and bottom row, respectively.}
  \end{center}


\end{figure}



\begin{figure}[t]
  \begin{center}
    \begin{tabular}{ccc}
      \begin{overpic}[width=.34\columnwidth]{%,grid]{
      {plots/LDP_prj_chunk_eps=4.0_d=32}.pdf}
      \end{overpic} &
      \hspace{-1cm}
      \begin{overpic}[width=.34\columnwidth]{%,grid]{
    {plots/LDP_prj_chunk_eps=8.0_d=32}.pdf}
      \end{overpic} &
      \hspace{-1cm}
      \begin{overpic}[width=.34\columnwidth]{%,grid]{
	  {plots/LDP_prj_chunk_eps=16.0_d=32}.pdf}
      \end{overpic}
      \\
      (a) & (b)  & (c)
    \end{tabular}
    %\caption{\label{fig:rand-proj} Performance of Projection-based algorithms with random projections and $d=32$.}
  \end{center}

  \begin{center}
    \begin{tabular}{ccc}
      \begin{overpic}[width=.34\columnwidth]{%,grid]{
      {plots/LDP_prj_chunk_eps=4.0_d=64}.pdf}
      \end{overpic} &
      \hspace{-1cm}
      \begin{overpic}[width=.34\columnwidth]{%,grid]{
    {plots/LDP_prj_chunk_eps=8.0_d=64}.pdf}
      \end{overpic} &
      \hspace{-1cm}
      \begin{overpic}[width=.34\columnwidth]{%,grid]{
	  {plots/LDP_prj_chunk_eps=16.0_d=64}.pdf}
      \end{overpic}
      \\
      (a) & (b)  & (c)
    \end{tabular}
    \caption{\label{fig:rand-proj} Performance of Projection-based algorithms with chunk-based random projections for $d=32$ and $d=64$ in the top and bottom row, respectively.}
  \end{center}


\end{figure}

\clearpage
\section{Optimality of $k$-random projections with $\privunit_\infty$}

Motivated by the previous experiments, here we try to prove optimality of the projection-based algorithm which used $k$ random vectors then privatizes the signs using $\privunit_\infty$. As we see in the empirical results, we expect the error to decompose into projection and privacy error and that the projection error becomes negligible for some $k \ge C \diffp$.

We briefly recall the algorithm here. Given input $v \in \sphere_2^d$, we have
\begin{enumerate}
    \item Draw $u_1,\dots,u_k \simiid \mathsf{Unif} (\sphere_2^d)$ (also orthogonal for now).
    \item Set $s_i = \mathsf{sign}(\<u_i,v\>)$
    \item Privatize $(\hat s_1,\dots,\hat s_k) = \privunit_\infty( s_1,\dots, s_k)$
    \item Return $\hat v = C \sum_{i=1}^k \hat s_i u_i$
\end{enumerate}

Here, letting $E^\star = \E_{u \sim \mathsf{Unif} (\sphere_2^d)}[| u_1 |]$,  the value of $C$ is 
\begin{align*}
    \frac{1}{C} 
        & = k \E_{u \sim \mathsf{Unif} (\sphere_2^d)}[u_1 \mid u_1 \ge 0] \\
        & = k E^\star \\
        & = k  \frac{2}{\sqrt{\pi}} \frac{\Gamma(\frac{d}{2}+1)}{d \Gamma(\frac{d-1}{2}+1)} \\
        & \approx \frac{k}{\sqrt{d}}.
\end{align*}

Let $\err_\infty(k,\diffp) = \E[\sum_{i=1}^k \hat s_i^2/k] = \E[\hat s_1^2]$.
The following theorem summarizes the guarantees of this algorithm. 
\begin{theorem}
    The $k$-random projection algorithm described above has as $d \to \infty$
    \begin{equation*}
    \E[\ltwo{\hat v}^2] 
        \to \begin{cases}
           \frac{\pi}{2} \frac{d}{k} \err_\infty(k,\diffp) & \text{if } c \diffp \le  k \\
           \frac{\pi}{2} \frac{d}{k}  & \text{Otherwise }
           \end{cases}
    \end{equation*}
\end{theorem}
\begin{proof}
    As the $u_i$'s are orthogonal, we have
    \begin{align*}
    \E\left[\ltwo{\hat v}^2 \right]
        & =  \E\left[\ltwo{C \sum_{i=1}^k \hat s_i u_i}^2 \right] \\
        & =  C^2 \E\left[ \sum_{i=1}^k \hat s_i^2 \right] \\
        & =  C^2 k \E\left[ \hat s_1^2 \right] \\
        & = \frac{\E\left[ \hat s_1^2 \right]}{ k \E_{u \sim \mathsf{Unif} (\sphere_2^d)}[| u_1 |]^2}.
    \end{align*}
    Note now that the guarantees of $\pu_\infty$ say that $\E[\hat s_1^2] = O(k/\diffp)$ for $\diffp \le k$. But note as well that $\E[\hat s_1^2] \ge 1$ as $\E[\hat s_1] = \E[s_1] \in \{-1,+1\}$. The claim now follows since $\E_{u \sim \mathsf{Unif} (\sphere_2^d)}[| u_1 |]^2  \to \frac{2}{\pi d}$
\end{proof}

\ha{I think we may be able to show that for $k \ge \diffp \log d$ and $\diffp = O(1)$, as $d \to \infty$ we have
\begin{equation*}
    \err_\infty(k,\diffp) 
        \le \frac{k}{d} \err_\infty(d,\diffp) 
        \le \frac{k}{d} \err_2(d,\diffp).
\end{equation*}
Overall this shows that for $k \ge \diffp \log d$
\begin{equation*}
    \err(\mathsf{k{-}proj}) \le  \frac{\pi}{2} \err(\pu_2).
\end{equation*}
}

\newcommand{\errproj}{\mathsf{ErrProj}}
\newcommand{\errpriv}{\mathsf{ErrPriv}}
Let us now consider the error of this algorithm. Noting that $\E[\hat s_i] = s_i$, we have
\begin{align*}
    \E\left[\ltwo{\hat v - v}^2 \right]
        & =  \E\left[\ltwo{C \sum_{i=1}^k \hat s_i u_i - v}^2 \right] \\
        & =  \E\left[\ltwo{C \sum_{i=1}^k \hat s_i u_i - C \sum_{i=1}^k  s_i u_i + C \sum_{i=1}^k  s_i u_i - v}^2 \right] \\
        & =  \E\left[\ltwo{C \sum_{i=1}^k \hat s_i u_i - C \sum_{i=1}^k  s_i u_i}^2\right]  + \E\left[\ltwo{C \sum_{i=1}^k  s_i u_i - v}^2 \right] \\
        & = \errpriv + \errproj.
\end{align*}

We will analyze each of these two errors separately. We assume without loss of generality that $v = e_1$ as the algorithm is invariant to rotations (\ha{maybe show more carefully}). Starting with the projection error $\errproj$, as $\E[C \sum_{i=1}^k  s_i u_i ] = v$ and $\< u_i, u_j\>=0$ we have
\begin{align*}
    \errproj
        & = \E\left[\ltwo{C \sum_{i=1}^k  s_i u_i - v}^2 \right] \\
        & = \E\left[\ltwo{C \sum_{i=1}^k  s_i u_i}^2 \right] - 1 \\
        & = C^2 \sum_{i=1}^k \E\left[\ltwo{u_i}^2 \right] + C^2 \E\left[\sum_{i \neq j} s_i s_j \< u_i, u_j\> \right] - 1 \\
        & = C^2 k - 1  \\
        & = \frac{1}{k \E_{u \sim \mathsf{Unif} (\sphere_2^d)}[| u_1 |]^2 } - 1 \\
        &  = \frac{{\pi}}  {4 k}\frac{d^2 \Gamma^2(\frac{d-1}{2}+1)} {\Gamma^2(\frac{d}{2}+1)} - 1 \\
        & \approx \frac{C d}{k} - 1
\end{align*}

As we know that the optimal error is at least $\frac{C_1 d}{\diffp}$, we have that $\errproj$ is smaller than the optimal error for some $k \ge C_2 \diffp$.

It remains to upper bound the privacy error $\errpriv$. We have
\begin{align*}
    \errpriv 
        & =  \E\left[\ltwo{C \sum_{i=1}^k \hat s_i u_i - C \sum_{i=1}^k  s_i u_i}^2\right] \\
        & =  \E\left[\ltwo{C \sum_{i=1}^k u_i (\hat s_i  - s_i) }^2\right] \\
        & =  C^2 k \E\left[|{\hat s_1  - s_1 }|^2\right] \\
        & = \frac{ \E\left[|{\hat s_1  - s_1 }|^2\right]}{k \E_{u \sim \mathsf{Unif} (\sphere_2^d)}[| u_1 |]^2}.
\end{align*}

Note that overall we have
\begin{align}
\label{eqn:error-main}
    \errpriv + \errproj
         & =  \frac{ \E\left[|{\hat s_1  - s_1 }|^2\right] + 1}{k \E_{u \sim \mathsf{Unif} (\sphere_2^d)}[| u_1 |]^2} - 1 \nonumber\\
         & = \frac{ \E\left[{\hat s_1^2}\right]}{k \E_{u \sim \mathsf{Unif} (\sphere_2^d)}[| u_1 |]^2} - 1. 
\end{align}

The goal is to prove that this error is less than the error of $\privunit_2$. It turns out we can connect this to the ratio of the optimal errors in $\ell_2$ and $\ell_\infty$ geometries. We denote the optimal error in $\ell_\infty$ geometry to be
\begin{equation*}
    \err(\ell_\infty) = \min_{\hat v: \text{unbiased }  \diffp \text{-DP}} \sup_{v \in \frac{1}{\sqrt{d}} \sphere_\infty^d} \E[\ltwo{\hat v}^2]
\end{equation*}
Similarly the error in $\ell_2$-geometry is $\err(\ell_2)$.  For $k=d$, in this terminology~\Cref{eqn:error-main} now becomes
\begin{align*}
    \frac{ \E\left[{\hat s_1 }^2\right]}{k \E_{u \sim \mathsf{Unif} (\sphere_2^d)}[| u_1 |]^2}
         & = \frac{ \E\left[(\frac{\hat s_1}{\sqrt{k}})^2 \right] }{\E_{u \sim \mathsf{Unif} (\sphere_2^d)}[| u_1 |]^2} \\
         & = \frac{\err(\ell_\infty)/k}{\E_{u \sim \mathsf{Unif} (\sphere_2^d)}[| u_1 |]^2} .
\end{align*}
The main goal is to prove that this error is less than $\err(\ell_2)$. Equivalently, as $\E_{u \sim \mathsf{Unif} (\sphere_2^d)}[| u_1 |] \to   \sqrt{\frac{2}{{\pi}}} \frac{1}{\sqrt{d}} $ for large $d$ (see below), this boils down to proving that (for $k=d$) 
\begin{align}
\label{eqn:err2_err_inf_ratio}
   \frac{\err(\ell_\infty) }{\err(\ell_2)} 
   \le d ~ \E_{u \sim \mathsf{Unif} (\sphere_2^d)}[| u_1 |]^2
   \to \frac{2}{\pi}.
\end{align}
Another way of writing this which may turn out to be useful is the following. Let $\hat v$ be the optimal estimator for $\ell_2$ and $\hat u$ be the optimal for $\ell_\infty$. Then we need to prove
\begin{align*}
   \E_{u \sim \mathsf{Unif} (\frac{1}{\sqrt{d}} \sphere_\infty^d)}[| u_1 |]^2 \E[\hat u_1^2]
   \le \E_{u \sim \mathsf{Unif} (\sphere_2^d)}[| u_1 |]^2 \E[\hat v_1^2].
\end{align*}
In other words, 
\begin{align*}
   \frac{\E[\hat u_1^2]}{\E[\hat v_1^2]}
   \le \frac{\E_{u \sim \mathsf{Unif} (\sphere_2^d)}[| u_1 |]^2}{\E_{u \sim \mathsf{Unif} (\frac{1}{\sqrt{d}} \sphere_\infty^d)}[| u_1 |]^2 } .
\end{align*}
\ha{Can we prove any of these? Note that~\Cref{eqn:error-main} immediately gives a sub-optimality ratio of $\frac{\pi}{2}$. Can we tighten this to $1$?}

\Cref{fig:err2-vs-err-inf} seems to be suggesting that this conjecture is indeed true. It only remains to prove it :)

\begin{figure}[t]
  \begin{center}
    \begin{tabular}{c}
      \begin{overpic}[width=.7\columnwidth]{%,grid]{
      {plots/err2_vs_err_inf_d=64}.pdf}
      \end{overpic} 
      \hspace{-1cm}
    \end{tabular}
     \caption{\label{fig:err2-vs-err-inf} Plotting the error of $\privunit_2$ normalized by $c$ (from~\Cref{eqn:err2_err_inf_ratio}) and the error of $\privunit_\infty$}
  \end{center}
\end{figure}

\subsection{Calculating  $\E_{u \sim \mathsf{Unif} (\sphere_2^d)}[| u_1 |] $}
It looks like we need to understand the quantity  $\E_{u \sim \mathsf{Unif} (\sphere_2^d)}[| u_1 |]^2$. First, we know that for $n \to \infty$ we have
$\Gamma(n+\alpha) = \Gamma(n) n^\alpha$ therefore we expect assuming $d/2 = \ell$
\begin{align*}
    \E_{u \sim \mathsf{Unif} (\sphere_2^d)}[| u_1 |] 
        & = \frac{2}{\sqrt{\pi}} \frac{\Gamma(\frac{d}{2}+1)}{d \Gamma(\frac{d-1}{2}+1)} \\
        & = \frac{2}{\sqrt{\pi} d} \frac{\Gamma(\ell+1)}{\Gamma(\ell+1/2)} \\
        & \to \frac{2 \sqrt{\ell} }{\sqrt{\pi} d } \\
        & = \sqrt{\frac{2}{{\pi}}} \frac{1}{\sqrt{d}}.
\end{align*}
Can we do this calculation more precisely?
Note that we have
\begin{equation*}
     \E_{u \sim \mathsf{Unif} (\sphere_2^d)}[| u_1 |] = \frac{2}{\sqrt{\pi}} \frac{\Gamma(\frac{d}{2}+1)}{d \Gamma(\frac{d-1}{2}+1)}.
\end{equation*}
We use properties of the Gamma functions, that is, for integer $n$
\begin{align*}
     \Gamma(n) & = (n-1)! \\
     \Gamma(n + {1}/{2}) & = \frac{(2n)!}{4^n n!} \sqrt{\pi}
\end{align*}
Assuming $d/2 = \ell$, we have
\begin{align*}
    \frac{\Gamma(\frac{d}{2}+1)}{\Gamma(\frac{d-1}{2}+1)}
         & = \frac{\Gamma(\ell+1)}{\Gamma(\ell+1/2)} \\
         & = \frac{(\ell!)^2 4^\ell }{(2\ell)! \sqrt{\pi}}
\end{align*}


\begin{remark}
    Some interesting observations from last meeting:
    \begin{enumerate}
        \item Maybe we can show that $\pug_2$ has the same error as $\pu_2$ which is easier to analyze (probably). Then we can similarly develop a $\pug_\infty$ and analyze that error and show it's error is similar to $\pu_\infty$. Finally, we only need to compare the errors of $\pug_\infty$ and $\pug_2$.
        \item Similar constant optimality for other problems. One example: stochastic optimization with unbiased minimizers. We expect that the optimal minimizers should be unbiased for strongly convex functions. This may allow to prove tight lower bounds in this setting too.
    \end{enumerate}
\end{remark}




\section{Analyzing $\pug_2$}
Let us introduce $\pug_2$. For a given $v \in \sphere_2^d$, we set \ha{maybe the orthogonal gaussian vector has to be normalized by $\sqrt{1-\alpha^2}$? though this will make privacy proof a bit more complicated..}
\begin{equation*}
    \hat v = \pug_2(v) = C \left(\alpha v + \normal(0,\sigma^2 (I - vv^T)) \right),
\end{equation*}
where $\sigma = \frac{1}{\sqrt{d}}$ and for $U \sim \normal(0,\sigma^2)$ we have
\begin{equation*}
    \alpha \sim 
    \begin{cases}
        U \mid U \ge \tau & \textit{w.p. } p \\
        U \mid U \le \tau & \textit{w.p. } 1 - p
    \end{cases}
\end{equation*}
To make $\pug_2$ unbiased, we set $C = 1/\E[\alpha]$.

Letting $\Phi_{\sigma^2}(\tau) = P(\normal(0,\sigma^2) \le \tau)$ denote the CDF of a Gaussian,  
we have the following guarantees for $\pug_2$.
\begin{theorem}
    Let $\diffp = \diffp_0 + \diffp_1$. Setting $p = \frac{e^{\diffp_0}}{e^{\diffp_0} + 1}$ and $\tau = \Phi_{\sigma^2}^{-1}(\frac{e^{\diffp_1}}{e^{\diffp_1} + 1}) = \sigma \cdot \Phi^{-1}(\frac{e^{\diffp_1}}{e^{\diffp_1} + 1})$, the algorithm $\pug_2$ is $\diffp$-DP. Moreover, it is unbiased and has error
    \begin{equation*}
        \E[\ltwo{\pug_2(v) - v}^2] =  \frac{\E [\alpha^2] + \frac{d-1}{d}}{\E[\alpha]^2} - 1.
    \end{equation*}
\end{theorem}

\begin{proof}
    We begin with the second part of the claim. $\pug_2$ is clearly unbiased and therefore
    \begin{equation*}
    \E[\ltwo{\pug_2(v) - v}^2] 
        =  \E[\ltwo{\pug_2(v)}^2] - 1
        = C^2 \left( \E [\alpha^2] + \frac{d-1}{d} \right) - 1
    \end{equation*}
    Now we proceed to prove the privacy claim. We need to show that for every $v_1,v_2 \in \sphere_2^d$ and $u \in \r^d$
    \begin{equation*}
        \frac{\pdf_{\pug(v_1)}(u)}{\pdf_{\pug(v_2)}(u)} \le e^\diffp.
    \end{equation*}
    One can show that the worst case for privacy is when $v_1$ and $v_2$ are orthogonal (\ha{show that}). In that case, we can for simplicity assume that $v_1 = e_1$ and $v_2 = e_2$. For this case, the ratio is maximized when $u_1 \ge \tau$ and $u_2 \le \tau$ for which we get
    \begin{align*}
    \log \frac{\pdf_{\pug(v_1)}(u)}{\pdf_{\pug(v_2)}(u)}
        & = \log \frac{\pdf_\alpha(u_1) }{\pdf_\normal(u_1) } + \log \frac{ \pdf_\normal(u_2)}{ \pdf_\alpha(u_2)} \\
        & = \log \frac{p}{P(U \ge \tau)} + \log \frac{P(U \le \tau)}{1-p} \\
        & = \log \frac{p}{1-p} + \log \frac{\Phi(\tau)}{1 - \Phi(\tau)} \\
        & = \diffp_0 + \diffp_1 \le \diffp.
    \end{align*}
    
\end{proof}



Our goal is now to show that the error of $\pug_2$ and $\pu_2$ is the same up to low order terms. To this end, note that
\begin{align*}
        \E[\ltwo{\pug_2(v) - v}^2] 
        & =  \frac{(\E [\alpha^2]-1/d) + 1}{\E[\alpha]^2} - 1 \\
        & =   \frac{(\E [\alpha^2]-1/d)}{\E[\alpha]^2} + \frac{1}{\E[\alpha]^2} - 1.
\end{align*}
We can show that $\E [\alpha^2]-1/d = O(1/d + \tau \log d)$ therefore this term is of lower order if $\tau = o(1/\log(d))$. For the second term, we need to show that
\begin{equation}
    | \E[U \mid U \ge \tau] - \E[W \mid W \ge \tau] | = o(\frac{\diffp}{d}),
\end{equation}
where $U \sim \normal(0,\sigma^2)$ and $W$ is the first coordinate of a uniform random vector over the sphere.

Note that we know~\cite[Inequality (1)]{DiaconisFr87}
\begin{equation}
    \norm{P_U - P_W}_{TV} \le \frac{8}{d-4}.
\end{equation}


% Note that for $X \sim \normal(\mu,\sigma^2)$, we have that 
% \begin{equation*}
%     \E[X \mid a \le X \le b]
%          = \mu - \sigma^2 \frac{\pdf(b) - \pdf(a)}{\Phi(b) - \Phi(a)}.
% \end{equation*}

For $X \sim \normal(\mu,\sigma^2)$ we have (see also inverse Mills ratio)
\begin{equation*}
    \E[U \mid U \ge \tau]
         %= 0 - \sigma^2 \frac{0 - \pdf(\tau)}{1 - \Phi(\tau)}
         =  \frac{\sigma^2 \pdf(\tau)}{P(U \ge \tau)}
\end{equation*}
and
\begin{equation*}
    \E[U \mid U \le \tau]
        % = 0 - \sigma^2 \frac{\pdf(\tau) }{ \Phi(\tau)}
         =  \frac{-\sigma^2 \pdf(\tau)}{P(U \le \tau)}
\end{equation*}
Overall we have that

\begin{align*}
    \E[\alpha]
        & = p \frac{\sigma^2 \pdf(\tau)}{P(U \ge \tau)} - (1-p) \frac{\sigma^2 \pdf(\tau)}{P(U \le \tau)} \\
        & = \sigma^2 \pdf(\tau) \left(\frac{p}{1 - P(U \le \tau)}  - \frac{1-p}{P(U \le \tau)} \right)
\end{align*}



To facilitate notation, given $p$ and $\gamma$, let $\diffp_2(p,\gamma)$ and $\err_2(p,\gamma)$ denote the privacy and (non-squared) error of $\privunit_2(p,\gamma)$. Similarly define $\diffp_G(p,\gamma)$ and $\err_G(p,\gamma)$.
We are now ready to prove the following theorem.
\begin{theorem}
    Let $p \in [0,1]$ and $\gamma \in [0,1]$. Then we have
    \begin{align*}
        \err_G(p,\gamma) & \le \err_2(p,\gamma)\left( 1  +  O\left(\frac{\sqrt{\log d}}{d} + \frac{e^\diffp +1}{d(e^\diffp -1)}) +  \gamma + \sqrt{\frac{\diffp_G + \log d}{d} } \right) \right)  \\
        \diffp_G(p,\gamma) & \le  \diffp_2(p,\gamma) + O \left( \frac{e^{\diffp_2(p,\gamma)}}{d} \right).
    \end{align*}
    In particular, for $\gamma \le O(\sqrt{\diffp/d})$ we have
   \begin{align*}
        \err_G(p,\gamma) & \le \err_2(p,\gamma)\left( 1  + O\left(\frac{\sqrt{\log d}}{d} + \frac{1}{d \min(\diffp,1)} +  \sqrt{\frac{\diffp + \log d}{d}} \right) \right) 
    \end{align*}
    % \ha{for privacy, we can also show:
    % \begin{equation*}
    %     \diffp_G(p,\gamma)
    %     \le \log(e^{\diffp_2(p,\gamma)} + O(1/d)).
    % \end{equation*}
    % }
\end{theorem}

\begin{proof}
    We make notation more concise by dropping $p$ and $\gamma$, this is, we will use $\diffp_G$ instead of $\diffp_G(p,\gamma)$.
    Let us start with the claim about privacy. Set $q_2 = P(W \le \gamma)$ and note that
    \begin{equation*}
    \diffp_2 
        = \log \frac{p}{1-p} + \log \frac{q_2}{1-q_2} 
        = \diffp_{2,0} + \diffp_{2,1},
    \end{equation*}
    where $W=Z_1$ for $Z \sim \mathsf{Unif}(\sphere_2^d)$. Moreover, for $q_G = P(U \le \gamma)$
    \begin{equation*}
    \diffp_G 
        = \log \frac{p}{1-p} + \log \frac{q_G}{1 - q_G} 
        = \diffp_{G,0} + \diffp_{G,1},
    \end{equation*}
    where $U \sim \normal(0,1/d)$. 
    % Thus it is enough to prove that 
    % \begin{equation*}
    %   \diffp_{G,1} \le  \diffp_{2,1} + \frac{1}{e^{\diffp_{2,1}}d}.   
    % \end{equation*}
    % Note that
    % \begin{align*}
    % | \frac{q_G}{1 - q_G} - \frac{q_2}{1-q_2}|
    %     & = \frac{|q_G - q_2|}{(1 - q_G)(1 - q_2)}
    % \end{align*}
    Thus it is enough to prove that 
    \begin{equation*}
      \diffp_{G,1} \le  \diffp_{2,1} + \frac{e^{\diffp_{2,1}}}{d}.   
    \end{equation*}
    Since $P(U \le \gamma) \le  P(W \le \gamma) + \frac{8}{d-4}$~\cite[Inequality (1)]{DiaconisFr87} and the function $\frac{q}{1-q}$ is increasing for $q \in (0,1)$ we have
    \begin{align*}
    \frac{P(U \le \gamma)}{1 - P(U \le \gamma)}
        & \le \frac{P(W \le \gamma) + 8/(d-4)}{1 - P(W \le \gamma) - 8/(d-4)} \\
        & = \frac{ \frac{e^{\diffp_{2,1}}} {e^{\diffp_{2,1}} + 1} + \frac{8}{d-4} }{\frac{1}{e^{\diffp_{2,1}}} - \frac{8}{d-4} }.
    \end{align*}
    Simple calculations show that the above term is smaller than $e^{\diffp_{2,1} + \rho}$ for $\rho = O(e^{\diffp_{2,1}}/d)$.
    
    Now we prove the claim about utility. Note that we can write for $q_2 = P(W \le \gamma)$
    \begin{align*}
    m_2(p,\gamma) 
        & = \E[W \indic{W \ge \gamma }] \frac{p+q_2-1}{q_2(1-q_2)}  \\
        %= \E[W \indic{W \le \gamma }] \frac{1-2p}{q} \\
    \err_2^2(p,\gamma) & = \frac{1}{m_2^2}    
    \end{align*}
    Similarly 
    \begin{align*}
    m_G(p,\gamma) 
        & = \E[U \indic{U \ge \gamma }] \frac{p+q_G-1}{q_G(1-q_G)} \\
        %= \E[U \indic{U \le \gamma }] \frac{p+q+1}{q(} \\
    \err_G^2(p,\gamma) & = \frac{\E[\alpha^2]-1/d}{m_G^2} + \frac{1}{m_G^2}  
    \end{align*}
    Now we have
    \begin{align*}
    \frac{\err_G}{\err_2}
        & \le \frac{m_2}{m_G} \sqrt{1 + \E[\alpha^2]} \\
        & = \frac{\E[W \indic{W \ge \gamma }]}{\E[U \indic{U \ge \gamma }]} \frac{p + q_G - 1}{q_G(1-q_G)} \frac{q_2(1-q_2)}{p + q_2 - 1} \sqrt{1 + \E[\alpha^2]} \\
        & \stackrel{(i)}{\le} (1 + \frac{ O(\frac{\sqrt{\log d}}{d^{3/2}})}{\E[U \indic{U \ge \gamma }]}) (1 + \frac{e^\diffp +1}{d(e^\diffp -1)}) (1 + \sqrt{\E[\alpha^2]}) \\
        & \stackrel{(ii)}{\le} 1 + O\left(\frac{\sqrt{\log d}}{d} + \frac{e^\diffp +1}{d(e^\diffp -1)}) +  \sqrt{\gamma^2 + \frac{\diffp_G + \log d}{d} } \right) \\
        & \le 1 + O\left(\frac{\sqrt{\log d}}{d} + \frac{e^\diffp +1}{d(e^\diffp -1)}) +  \gamma + \sqrt{\frac{\diffp_G + \log d}{d} } \right),
        % & \le (1 + \frac{ O(\frac{\sqrt{\log d}}{d^{3/2}})}{\E[U \indic{U \ge \gamma }]}) (1 + \frac{e^\diffp +1}{d(e^\diffp -1)}) (1 + \sqrt{\E[\alpha^2]}) \\
        % & \le \frac{m_G + O(\frac{\sqrt{\log d}}{d^{3/2}}) }{m_G} (1 + \sqrt{\E[\alpha^2]}) \\
        % & \le (1 + \frac{O(\sqrt{\log d}}{d \sqrt{\diffp}}) (1 + \sqrt{\E[\alpha^2]}) \\
        % & \le 1 + O \left(\frac{\sqrt{\log d}}{d \sqrt{\diffp}} +\sqrt{\gamma^2 + \frac{\diffp_G + \log d}{d} } \right) ,
    \end{align*}
    where $(i)$ follows from~\Cref{lemma:bound-diff-exp}, \Cref{lemma:bound-ratio-q} and~\Cref{lemma:bound-sec-moment} and $(ii)$ follows since $\E[U \indic{U \ge \gamma }] \ge \E[U \indic{U \ge 0}] = \E[|U|]/2 \ge \Omega(\sigma) = \Omega(1/\sqrt{d}) $.
    
    
    
    % First, Lemma~\ref{lemma:bound-sec-moment} gives that $\E[\alpha^2] = O \left( \gamma^2 + \frac{\diffp_G + \log d}{d} \right)$ \ha{need to fix some issues here..}. Moreover, as $|2p-1| \le 1$ and $q \in [0,1]$, we have that
    % \begin{equation*}
    % |m_G(p,\gamma) - m_2(p,\gamma) |
    %     \le 2 \max\left(|\E[W \indic{W \ge \gamma }] - \E[U \indic{U \ge \gamma }]|, |\E[W \indic{W \le \gamma }] - \E[U \indic{U \le \gamma }]| \right)
    % \end{equation*}
    % We will upper bound the first term in the maximum; bounding the other term follows from identical arguments. We have
    % \begin{align*}
    % |\E[W \indic{W \ge \gamma }] - \E[U \indic{U \ge \gamma }]|     & = |\int_{\gamma}^\infty u (\pdf_W(u) - \pdf_U(u)) du| \\
    %   & \le | \int_{\gamma}^C u (\pdf_W(u) - \pdf_U(u)) du|  + | \int_{C}^\infty u (\pdf_W(u) - \pdf_U(u)) du| \\
    %   & \le C \norm{P_W - P_U}_{TV} + \int_{C}^1 u \pdf_W(u) du + \frac{\pdf_U(C)}{d} \\
    %   & \le \frac{8C}{d-4} + \frac{e^{-C^2 d/2}}{\sqrt{2 \pi d}} + \pdf_W(C) \\
    %   & \stackrel{(i)}{\le} \frac{8C}{d-4} + \frac{e^{-C^2 d/2}}{\sqrt{2 \pi d}} + O(\sqrt{d} e^{-C^2 d/8}) \\
    %   & \le O(\frac{\sqrt{\log d}}{d^{3/2}}).
    % \end{align*}
    % where the last inequality follows by setting $C = \Theta(\sqrt{\frac{\log(d)}{d}})$. Before proving inequality $(i)$, we can now finish the proof. Indeed we have
    % \begin{align*}
    % \frac{\err_G}{\err_2}
    %     & \le \frac{m_2}{m_G} \sqrt{1 + \E[\alpha^2]} \\
    %     & \le \frac{m_G + O(\frac{\sqrt{\log d}}{d^{3/2}}) }{m_G} (1 + \sqrt{\E[\alpha^2]}) \\
    %     & \le (1 + \frac{O(\sqrt{\log d}}{d \sqrt{\diffp}}) (1 + \sqrt{\E[\alpha^2]}) \\
    %     & \le 1 + O \left(\frac{\sqrt{\log d}}{d \sqrt{\diffp}} +\sqrt{\gamma^2 + \frac{\diffp_G + \log d}{d} } \right) ,
    % \end{align*}
    % where the second inequality follows by noticing that existing lower bounds imply  $\err_2(p,\gamma) \ge 1/m_G \ge \Omega(\sqrt{d/\diffp})$.
    
    % Inequality $(i)$ follows since $W$ has the same distribution as $2B-1$ for $B \sim \mathsf{Beta}(\frac{d-1}{2},\frac{d-1}{2})$. Indeed setting $\alpha = \frac{d-1}{2}$, we have for any $b = 1/2 + \rho$
    % \begin{align*}
    % \pdf_B(b)
    %      & = \frac{(b(1-b))^{\alpha-1}}{B(\alpha,\alpha)} \\
    %      & = \frac{(1-\rho^2)^{\alpha-1}}{4^{\alpha-1}} \frac{1}{B(\alpha,\alpha)} \\
    %      & \le \frac{e^{-\rho^2(\alpha-1)}}{4^{\alpha-1}} \frac{1}{B(\alpha,\alpha)} \\
    %      & \le O(\sqrt{\alpha} e^{-\rho^2\alpha}),
    % \end{align*}
    % where the last inequality follows from
    % \begin{align*}
    % B(\alpha,\alpha)
    %      = \frac{2}{\alpha} \frac{1}{\binom{2\alpha}{\alpha}} 
    %     \ge \frac{2}{\alpha} \Omega(\frac{\sqrt{\alpha}}{4^\alpha}) 
    %     = \Omega(\frac{1}{\sqrt{\alpha} 4^\alpha}) .
    % \end{align*}
    % The claim now follows as $\pdf_W(C) = \pdf_B(1/2 + C/2)$.
\end{proof}


\begin{lemma}
\label{lemma:bound-diff-exp}
    We have
    \begin{equation*}
    |\E[W \indic{W \ge \gamma }] - \E[U \indic{U \ge \gamma }]|     
        \le O\left(\frac{\sqrt{\log d}}{d^{3/2}}\right).
    \end{equation*}
\end{lemma}
\begin{proof}
    We have
    \begin{align*}
    |\E[W \indic{W \ge \gamma }] - \E[U \indic{U \ge \gamma }]|     & = |\int_{\gamma}^\infty u (\pdf_W(u) - \pdf_U(u)) du| \\
       & \le | \int_{\gamma}^C u (\pdf_W(u) - \pdf_U(u)) du|  + | \int_{C}^\infty u (\pdf_W(u) - \pdf_U(u)) du| \\
       & \le C \norm{P_W - P_U}_{TV} + \int_{C}^1 u \pdf_W(u) du + \frac{\pdf_U(C)}{d} \\
       & \le \frac{8C}{d-4} + \frac{e^{-C^2 d/2}}{\sqrt{2 \pi d}} + \pdf_W(C) \\
       & \stackrel{(i)}{\le} \frac{8C}{d-4} + \frac{e^{-C^2 d/2}}{\sqrt{2 \pi d}} + O(\sqrt{d} e^{-C^2 d/8}) \\
       & \le O(\frac{\sqrt{\log d}}{d^{3/2}}).
    \end{align*}
    where the last inequality follows by setting $C = \Theta(\sqrt{\frac{\log(d)}{d}})$.
    Inequality $(i)$ follows since $W$ has the same distribution as $2B-1$ for $B \sim \mathsf{Beta}(\frac{d-1}{2},\frac{d-1}{2})$. Indeed setting $\alpha = \frac{d-1}{2}$, we have for any $b = 1/2 + \rho$
    \begin{align*}
    \pdf_B(b)
         & = \frac{(b(1-b))^{\alpha-1}}{B(\alpha,\alpha)} \\
         & = \frac{(1-\rho^2)^{\alpha-1}}{4^{\alpha-1}} \frac{1}{B(\alpha,\alpha)} \\
         & \le \frac{e^{-\rho^2(\alpha-1)}}{4^{\alpha-1}} \frac{1}{B(\alpha,\alpha)} \\
         & \le O(\sqrt{\alpha} e^{-\rho^2\alpha}),
    \end{align*}
    where the last inequality follows from
    \begin{align*}
    B(\alpha,\alpha)
         = \frac{2}{\alpha} \frac{1}{\binom{2\alpha}{\alpha}} 
        \ge \frac{2}{\alpha} \Omega(\frac{\sqrt{\alpha}}{4^\alpha}) 
        = \Omega(\frac{1}{\sqrt{\alpha} 4^\alpha}) .
    \end{align*}
    The claim now follows as $\pdf_W(C) = \pdf_B(1/2 + C/2)$.
\end{proof}


\begin{lemma}
    \label{lemma:bound-ratio-q}
    We have
    \begin{equation*}
    \frac{p + q_G - 1}{q_G(1-q_G)}
    \frac{q_2(1-q_2)}{p + q_2 - 1}
        \le 1 + O\left(\frac{e^{\diffp} + 1}{d(e^{\diffp} - 1)} \right).
    \end{equation*}
\end{lemma}
\begin{proof}
    Note that if $q_G \le q_2$ then the ratio is less than $1$. Otherwise $q_2 \le q_G \le q_2 +1/d$. Note that
    \begin{align*}
    \frac{p + q_G - 1}{q_G(1-q_G)}
    \frac{q_2(1-q_2)}{p + q_2 - 1}
        & = \frac{p + q_G - 1}{p + q_2 - 1}
          \frac{q_2}{q_G} \frac{1-q_2}{1-q_G} \\
        & \le  \frac{p + q_2 + 1/d - 1}{p + q_2 - 1}
           \frac{1-q_G + 1/d}{1-q_G} \\
        & = (1 + \frac{1}{d(p + q_2 - 1)}) (1 + \frac{1}{d(1-q_G)}).
    \end{align*}
    Note that $q_G \ge e^{-\diffp}$ which implies that \begin{equation*}
    \frac{1}{1-q_G} \le \frac{e^\diffp + 1}{e^\diffp - 1}.
    \end{equation*}
    Moreover, assuming without loss of generality that $\diffp_{2,0} \le \diffp_{2,1}$, we get that $\diffp_{2,1} \ge \diffp/2$ and therefore as $p \ge 1/2$ we have 
    \begin{align*}
    \frac{1}{p + q_2 - 1}
        & \le  \frac{1}{q_2 - 1/2} \\
        & \le \frac{1}{e^{\diffp/2}/(e^{\diffp/2}+1) - 1/2} \\
        & = \frac{2 (e^{\diffp/2} + 1)}{e^{\diffp/2} - 1}.
    \end{align*}
    This proves the claim as $\frac{e^{\diffp} + 1}{d(e^{\diffp} - 1)} \le 1$.
\end{proof}


\begin{lemma}
\label{lemma:bound-sec-moment}
    We have
    \begin{equation*}
        \E[\alpha^2] \le O \left(\gamma^2 + \frac{\diffp_G + \log d}{d} \right).
    \end{equation*}
\end{lemma}
\begin{proof}
    It is enough to upper bound $\E[U^2 \mid U \ge \gamma]$. Since $P(U \ge \gamma) \ge e^{-\diffp_G}$
    \begin{align*}
    \E[U^2 \mid U \ge \gamma]
        & = \int_{\gamma}^C u^2 \frac{f_U(u)}{P(U \ge \gamma)} du + \int_{C}^\infty u^2 \frac{f_U(u)}{P(U \ge \gamma)} du \\
        & \le C^2 + e^{\diffp_G} \frac{1}{\sqrt{2\pi d}} \int_{C}^\infty u^2 de^{-u^2 d/2} du \\
        & \le  C^2  + e^{\diffp_G} \frac{e^{-C^2 d/4}}{\sqrt{2\pi d}} \int_{C}^\infty u^2 de^{-u^2 d/4} du \\ 
        & \le O \left(\gamma^2 + \frac{\diffp_G + \log d}{d} \right) ,
    \end{align*}
    where the last inequality follows by setting $C = \Theta\left( \max \left(\gamma, \sqrt{\frac{\diffp_G + \log d}{d}} \right) \right)$.
\end{proof}



\subsection{Comparing $\pug$ to $\pu_\infty$}

Note that the error of $\pug$ is $ \err_G(p,\gamma) = 1/m_G$ where $q = P(U \le \gamma)$ and
\begin{equation*}
    m_G(p,\gamma) 
        = \frac{p+q-1}{q(1-q)} \frac{\pdf_U(\gamma)}{d}.
\end{equation*}


For $\pu_\infty$ we can show that
\begin{equation*}
    m_\infty(p,\gamma) 
        = \frac{p+q_\infty-1}{q_\infty(1-q_\infty)} \frac{\binom{d-1}{\ceil{\frac{d + d\gamma +1}{2}}-1}}{2^d},
\end{equation*}
where $q_\infty = P(\frac{\sum_{i=1}^d W_i}{\sqrt{d}} \le \gamma) $ and $W_i \sim \uniform\{\frac{-1}{\sqrt{d}},\frac{1}{\sqrt{d}}\}$. Note that we also have
\begin{equation*}
    q_\infty 
        = P\left(\frac{\sum_{i=1}^d W_i}{\sqrt{d}} \le \gamma\right)
        = P\left( \mathsf{Bin}(d,\frac{1}{2}) \le \frac{d(1+\gamma)}{2} \right).
\end{equation*}

CLT theorem implies that $q_\infty \to q$. We can also show that for $\gamma \le \sqrt{\diffp/d}$ we have
\begin{equation*}
    \binom{d-1}{\ceil{\frac{d + d\gamma +1}{2}}-1}
        \to \frac{2^d e^{-d\gamma^2/2}}{\sqrt{2 \pi (d-1)}}.
\end{equation*}
which implies that 
\begin{equation*}
    \frac{\binom{d-1}{\ceil{\frac{d + d\gamma +1}{2}}-1}}{2^d} \frac{d}{\pdf_U(\gamma)} \to 1.
\end{equation*}
Unfortunately we don't get the $\sqrt{\pi/2}$ factor we want. Something wrong here? Or maybe we need different $p$ and $\gamma$ for $\pug_2$ and $\pu_\infty$? \textbf{NOTE} that maybe the problem is the approximation of the error here because the error of $\pug$ is not $1/m_G$ but depends on $\E[\alpha^2]$.




